Dynamic Defender-Attacker Blotto Game

This work studies a dynamic, adversarial resource allocation problem in environments modeled as graphs. A blue team of defender robots are deployed in the environment to protect the nodes from a red team of attacker robots. We formulate the engagement as a discrete-time dynamic game, where the robots can move at most one hop in each time step. The game terminates with the attacker's win if any location has more attacker robots than defender robots at any time. The goal is to identify dynamic resource allocation strategies, as well as the conditions that determines the winner: graph structure, available resources, and initial conditions. We analyze the problem using reachable sets and show how the outdegree of the underlying graph directly influences the difficulty of the defending task. Furthermore, we provide algorithms that identify sufficiency of attacker's victory.

==> propagation.tex <==
\section{Open-Loop Strategies via reachable Sets}
We first extend the definition of reachable set $\R(\x_t)$ of a single point $\x_t$ to the reachable set of a polytope. 
We consider the set of all possible states that can be reached in the next time step from the polytope $D_t \in \mathbb{R}^N$:
\begin{equation}\label{eqn:rechability-set}
    \R(D_t) = \left\{ \x_{t+1} \; \vert\; \exists K\in \K \text{ and } \x_t \in D_t \text{ such that } \x_{t+1} = \x_t  K \right\}.
\end{equation}
\begin{fact}
The set $\R(D_t)$ can be constructed as a union of the reachable sets of single points $\x_t \in D_t$ via:
\begin{equation*}
    \R(D_t) = \bigcup_{\x_t \in D_t} \R(\x_t).
\end{equation*}
\end{fact}

Suppose that the extreme points of the polytope $D$ are $\{\x_{D_t}^{(s)}\}_s$.  
Then all points $\x_{t+1}$ in $\R(D_t)$ can be represented as:
\begin{equation}\label{eqn:characterization-reachable-D}
    \x_{t+1} = \left(\sum_s \theta^{(s)} \x_{D_t}^{(s)} \right) \left(\sum_{\ell}\lambda^{(\ell)}\hatK^{(\ell)}\right)  = \sum_{\ell, s} \left(\theta^{(s)} \lambda^{(\ell)}\right) \left(\x_{D_t}^{(s)}\hatK^{(\ell)}\right).
\end{equation}
Consequently, the set $\R(D_t)$ is the convex hull of $\{\x_{D_t}^{(s)}\hatK^{(\ell)}\}_{\ell,s}$, and the vertices of $\R(D_t)$ is a subset of these points.

To obtain the open-loop strategies, we first propagate the safe sets in~\eqref{eqn:safe-set} and the reachable sets in~\eqref{eqn:rechability-set}.
With the flow of safe sets and the reachable sets, we can extract the open-loop policies for the agents.

\begin{algorithm}[h]
\SetAlgoLined
\SetKwInput{KwInputs}{Inputs}
\KwInputs{Trasversibility matrices $A^X, A^Y$; Initial states $\x_0, \y_0$, Terminal time $T_f$;}
Compute the extreme action sets $\hatcalK, \hatcalF$ via~\eqref{eqn:extreme-actions}\;
Set $D_0^X \leftarrow \{\x_0\}$ and $\R_0^Y \leftarrow \{\y_0\}$\;
 \For{t = 1 to $T_f$}{
  Propagate reachable set:
  $\R^X_{t} \leftarrow \R(D^X_{t-1})$,
  $\R^Y_{t} \leftarrow \R(\R^Y_{t-1})$ \;
  Compute $\x_{\req,t}$ via~\eqref{eqn:x_req} based on $\R^Y_{t}$\;
  Construct $\polytope_{\req,t}$ via~\eqref{eqn:poly_req}\; 
  Construct safe set for the Defender:
  $D^X_{t} \leftarrow \R^X_{t} \bigcap \polytope_{\req,t}$ \;
  \If{$D^X_{t}$ is empty}{
  \textbf{Return} set flow up to $t$: $\left\{D^X_{\tau}\right\}_{\tau=0}^t$, $\left\{\R^X_{\tau}\right\}_{\tau=0}^t$ and $\left\{\R^Y_{\tau}\right\}_{\tau=0}^t$\;
   }
 }
 \textbf{Return} set flow $\left\{D^X_{\tau}\right\}_{\tau=0}^{T_f}$, $\left\{\R^X_{\tau}\right\}_{\tau=0}^{T_f}$ and $\left\{\R^Y_{\tau}\right\}_{\tau=0}^{T_f}$\;
 \caption{Safe Set and Reachable Sets Propagation}
 \label{alg:set-prop}
\end{algorithm}

\begin{lemma}\label{lmm:reachable-set-lemma}
For any point $\x_t \in D^X_t$, there is a sequence of actions $\{K_\tau\}_{\tau=0}^{t-1}$ that take the Defender's state from $\x_0$ to $\x_t$, while guaranteeing $x_\tau \in D^X_{\tau}$ for all steps $\tau \leq t-1$.
\end{lemma}
\begin{proof}
We provide a proof by induction on $t$.
Consider the base case of $\x_1$. Since $\x_1 \in D_1^X \subset \R(\x_0)$, by the definition of $\R(\x_0)$, there exists an action $K_0$ such that $\x_1 = \x_0 K_0$ and $x_0 \in D^X_0$. So the base statement holds for $t=1$.

Suppose the statement holds for a given $t\geq 0$.
Consider a point $\x_{t+1} \in D^X_{t+1}$. 
By construction $D^X_{t+1} \subset \R(D^X_{t})$.
Thus, there exists a point $\x_t \in D^X_{t}$ and an action $K_t$, such that $\x_{t+1} = \x_t K_t$.
Due to the assumed statement, there is a sequence of actions $\{K_\tau\}_{\tau=0}^{t-1}$ that takes $\x_0$ to $\x_t$ while maintaining the whole trajectories within $\{D^X_\tau\}_\tau$.
Concatenate action $K_t$ to the this sequence and consider the fact that $x_t \in D^X_t$, we have shown that the statement in Lemma~\ref{lmm:reachable-set-lemma} holds for $t+1$, which concludes the proof.
\end{proof}

\begin{theorem}\label{thm:existence-of-defender-policy}
If Algorithm~\ref{alg:set-prop} returns a non-empty $D_{T_f}^X$, then there exists an open-loop Defender strategy $\left\{K^*_t\right\}_{t=0}^{T_f-1}$ such that for any Attacker's strategy $\left\{F_t\right\}_{t=0}^{T_f-1}$, the Defender can guard all locations at all time steps $t \leq T_f$.
\end{theorem}
\begin{proof}
Since $D_{T_f}^X$ is non-empty, we can pick a point $\x_{T_f} \in D_{T_f}^X$. Per Lemma~\ref{lmm:reachable-set-lemma}, there is a sequence of actions $\left\{K^*_t\right\}_{t=0}^{T_f -1}$ that takes $\x_0$ to $\x_{T_f}$.
Furthermore, this action sequence results in a trajectory $\{\x^*_t\}_{t=0}^{T_f}$ such that at each time step \mbox{$\x^*_t \in D^X_t$} for all $t=1,\ldots,T_f-1$.

Recall that the reachable set $\R_t^Y$ contains all the states $\y_t$ that the Attacker can achieve at time $t$ and the safe set $D^X_t$ is constructed based on $\R_t^Y$.
Consequently, for any point $\x_t \in D^X_t$, there is no Attacker state $\y_t$ that is reachable and also can terminate the game at $t$.

In summary, the open-loop Defender strategy $\left\{K^*_t\right\}_{t=0}^{T_f-1}$ can guard against all Attacker's admissible strategies up to $T_f$.
\end{proof}

\begin{remark}
The Defender's winning strategy $\left\{K^*_t\right\}_{t=0}^{T_f-1}$ and any Attacker strategy $\left\{F_t\right\}_{t=0}^{T_f-1}$ forms a Nash equilibrium for this ``game of kind" type sDABG.
For the Defender, it has no incentive to deviate, as it is already guaranteed to win against all Attacker's strategies. 
The Attacker, on the other hand, does not gain any performance by deviating from its current strategy, since no admissible strategy can beat the Defender's strategy $\left\{K^*_t\right\}_{t=0}^{T_f-1}$.
\end{remark}


\begin{theorem}\label{thm:existence-of-attacker-policy}
If Algorithm~\ref{alg:set-prop} returns $D_\tau^X = \emptyset$ at some $\tau \leq T_f$, then for any strategy $\left\{K_t\right\}_{t=0}^{\tau-1}$ that the Defender X may deploy, there is a counter strategy $\left\{F_t\right\}_{t=0}^{\tau-1}$ for the Attacker Y, such that at time step $\tau$, Y will win at least one node. 
\end{theorem}
\begin{proof}
Consider an arbitrary $\left\{K_t\right\}_{t=0}^{\tau-1}$ and its resulted state trajectory $\left\{\x_t\right\}_{t=0}^{\tau}$.
By the definition of $\polytope_{\req,t}$, for all $\x_t \notin \polytope_{\req,t}$, there exists a Attacker state $\y_t \in \R_t^Y$ such that the Attacker wins at that time step.

\textbf{Case 1:} $\x_t \notin D^X_t$ for some $t<\tau$, that is $\x_t \notin \polytope_{\req,t}$.
Then at $t$, there is a state $\y_t$ reachable such that the Attacker will win at least one location. 
The game terminates at $t$ with the Attacker's victory.

\textbf{Case 2:} $\x_t \in D^X_t$ for all $t<\tau$. Since $D^X_\tau$ is empty, we know that any $\x_\tau$ that is reachable at this time step cannot be in the set $\polytope_{\req,\tau}$.
Consequently, there exists a $\y^*_\tau \in \R^Y_t$ that Attacker can move to and win the game. 
Through a similar argument as in Theorem~\ref{thm:existence-of-defender-policy}, one can construct a strategy for the Attacker that will take $\y_0$ to $\y^*_\tau$, and this strategy will defeat the given Defender's strategy.
\end{proof}

Theorem~\ref{thm:existence-of-attacker-policy} states that if $D_\tau^X$ is empty, then regardless what strategy the Defender deploys, an \textit{omnipotent} Attacker that knows the Defender's strategy \textit{a priori} can find a counter-strategy and win the game no later than $\tau$ steps.
However, how to construct counter-strategy in this scenario without the knowledge of the Defender's strategy remains as a future research topic. 

\subsection{Policy Extractions}
\paragraph{Backward Propagation.}
An essential element of constructing policies from reachable sets is to find a state $\x_t \in D_t$ and an action $K_t$ that leads to a given state $\x_{t+1} \in \R(D_t)$.
By the construction of $\R(D_t)$, the existence of such state and admissible action is guaranteed. 
We show that such an $K_t$ can be found through a linear program.

Recall the characterization of $\R(D_t)$ in~\eqref{eqn:characterization-reachable-D}.
Specifically, if $\x_{t+1} \in \R(D_t)$, it satisfies
\begin{align}\label{eqn:back-prop-coeff}
    \x_{t+1} = \sum_{\ell, s} \left(\theta^{(s)} \lambda^{(\ell)}\right) \left(\x_{D_t}^{(s)}\hatK^{(\ell)}\right),
\end{align}
where $\left\{\x_{D_t}^{(s)}\right\}_s$ are the vertices of polytope $D_t$ and $\left\{\hatK^{(\ell)}\right\}_\ell$ are the extreme actions.
Furthermore, the action $K = \sum_{\ell} \lambda^{(\ell)} \hatK^{(\ell)}$ and the state $\x_t = \sum_{s} \theta^{(s)} x^{(s)}_{D_t}$ are the state and action pair that will lead to the given $\x_{t+1}$.
Thus, the problem is reduced to finding the convex coefficients that satisfies the constraints above.
We do a change of variables to make the problem linear by letting $\psi_{(s,\ell)} = \theta^{(s)}\lambda^{(\ell)}$, and we use $\bm{\psi}$ to denote the stacked vector.
Then, the problem above can be easily solved as finding \textit{a feasible solution} of the following linear program:
\begin{alignat}{2}
    &\max_{\bm{\psi}} \quad  && 0
    \label{eqn:lp-action-1}\\
    &\text{subject to } \qquad  && R \bm{\psi} = \x_{t+1}\trps
    \label{eqn:lp-action-2}\\
    &\quad                      && \sum_{\ell} \psi_{s,\ell} = 1 \quad \forall s 
    \label{eqn:lp-action-3}\\
    &\quad                      && \sum_{s} \psi_{s,\ell} = 1 \quad \forall \ell \label{eqn:lp-action-4}\\
    &\quad                      && \bm{\psi} \geq 0 \label{eqn:lp-action-5}
\end{alignat}
where the matrix $R$ in~\eqref{eqn:lp-action-2} has $\left(\x_{D_t}^{(s)} \hatK^{(\ell)}\right)\trps$ as its columns. 
The optimization objective in~\eqref{eqn:lp-action-1} is \textit{irrelevant}, as we are just seeking a feasible solution.
A feasible solution is guaranteed by the fact $\x_{t+1} \in \R(\x_t)$, and the original coefficients  $\bm{\lambda}$ and $\bm{\theta}$ in~\eqref{eqn:back-prop-coeff} can be reconstructed through a marginalization via
\begin{equation}\label{eqn:convex-reconstruct}
    \theta^{(s)} = \sum_{\ell} \psi_{s,\ell}, \qquad \lambda^{(\ell)} = \sum_s \psi_{s,\ell}.
\end{equation}
We use the function \textit{BackProp} to denote the operations above, and we summarize this function in Algorithm~\ref{alg:back-prop}.

\begin{algorithm}[h]
\SetAlgoLined
\SetKwInput{KwInputs}{Inputs}
\KwInputs{Start polytope $D_t$; end state $\x_{t+1}$}
Compute the vertices of the reachable set $\R(\x_{t})$ via~\eqref{eqn:characterization-reachable-D}\;
Form the matrix $R$ \;
Solve the linear program in~\eqref{eqn:lp-action-1} to~\eqref{eqn:lp-action-5}\;
Reconstruct the convex coefficients $\bm{\lambda}$ and $\bm{\theta}$ as in~\eqref{eqn:convex-reconstruct} \;
\textbf{Return} $K_t = \sum_{\ell} \lambda^{(\ell)} \hatK^{(\ell)}$ and $\x_t = \sum_{s} \theta^{(s)} \x^{(s)}_{D_t}$
\caption{BackProp}
\label{alg:back-prop}
\end{algorithm}



\paragraph{Non-empty Terminal Safe Set}
Suppose $D_{T_f}^X$ is not empty. 
We can extract the open-loop strategy of the Defender as follows:

\begin{algorithm}[h]
\SetAlgoLined
\SetKwInput{KwInputs}{Inputs}
\KwInputs{Reachable set flow $\left\{D^X_{t}\right\}_{t=0}^{T_f}$}
Pick a point $\x_{T_f} \in D^X_{T_f}$\;
\For{t= $T_f$ to 1}{
$\x_{t-1}, K^*_{t-1}$ $\leftarrow$ BackProp($D^X_{t-1}, \x_t$)
}
Return $\{x_t\}_{t=0}^{T_f}$ and $\{K^*_t\}_{t=0}^{T_f}$
\caption{Extract Defender Strategy}
\label{alg:defender-policy}
\end{algorithm}
Per Theorem~\ref{thm:existence-of-defender-policy}, the strategy  $\{K^*_t\}_{t=0}^{T_f}$ found by Algorithm~\ref{alg:defender-policy} can defend all Attacker's strategies. 


\paragraph{Empty Safe Set}
Suppose $D_{t}^X$ is empty for some $t \leq T_f$, then for all Defender's strategies, there is an Attacker's strategy that leads to Attacker's victory. 

\sg{Scott: I am stuck on how to generate the \textbf{closed-loop} strategy for the Attacker. Since we need to ensure that the $\y^*_t$ that will terminate the game is reachable at that time step. 
However, this requires adapting to the Defender's selection of state, and the Defender would also adapt accordingly, and now it really becomes a game.}


\clearpage
\begin{appendix}

\input{propagation}

\sg{Is there a motivation for the Attacker to split its resource?}

\todo{Theorem on splitting?}

\todo{Algorithm to find $\tau$?}

\section{Sub-game Decomposition}
\sg{Restricted Games and Sub-Game Equivalence}


\begin{definition}[Sub-games]
We say a game $G =\langle \graph^X, \graph^Y, \x_0, \y_0 \rangle$ can be decomposed into $m$ sub-games $ G^q=\langle \graph^X, \graph^Y, \x^{q}_0, \y^{q}_0 \rangle$ for $q=1,\ldots, m$, if 
\begin{equation*}
    \sum_{q} \x^{q}_0 = \x_0,~  \sum_{q}\y^q_0 = \y_0, \text{ and } \x^{q}_0 \geq \y^{q}_0 \;\forall \; q=1,\ldots, m.
\end{equation*}
\end{definition}

\daigo{I think the assumptions on the resources must be strengthened based on $X^q\geq \doutmax Y^q$}

\att{The original game is a subgame of itself. 
We need a definition of \textit{proper subgame}.
We also need a definition of minimal winning subgame, such that if any of the resource within this subgame is removed, the Attacker can no longer win the game. This will help us identify the most important part of the game.}

\begin{lemma}
Consider the sequence of actions $\left\{K^{q}_t\right\}_t$ deployed by the sub-Defender $q$ within sub-game $G^q$.
Then the $m$ sequences of actions deployed within each of the $m$ sub-games corresponds to a sequence of actions $\left\{K_t\right\}_t$ of the original game $G$.
Further more,
\begin{equation}
    [K_t]_{ij} = \sum_q \frac{[\x^q_t]_j}{[\x_t]_j}  [K_t^q]_{ij},
\end{equation}
where $[\x_t]_j = \sum_q [\x_t^q]_j$.
Similar results apply to the Attacker's side of the game.
\end{lemma}
\begin{proof}
Consider the states $(\x_t^1,\ldots, \x_t^m)$ of the $m$ sub-games  at time step $t$. This collection of sub-game states corresponds to the state of the original game $\x_t = \sum_{q=1}^{m} \x_t^q$.
Suppose the sub-defender $q$ applies an action $K_t^q$, then the new sub-game state is $\x^q_{t+1} = K_t^q \x^q_t$,
and the resulted original state from the $m$ sub-game states is given by
\begin{equation}
    \x_{t+1} = \sum_{q=1}^m K_t^q \x^q_t.
\end{equation}
More specifically, element-wise we have
\begin{align}
    [\x_{t+1}]_i &= \sum_{q=1}^m [K_t^q \x^q_t]_i = \sum_{q=1}^m \sum_{j=1}^{|\nodeset|} [K_t^q]_{ij} [\x^q_t]_j \\
    &=  \sum_{j=1}^{|\nodeset|} \left(\sum_{q=1}^m  \frac{[\x^q_t]_j}{[\x_t]_j} [K_t^q]_{ij}\right)[\x_t]_j \\
    &= \sum_{j=1}^{|\nodeset|} [K_t]_{ij} [\x_t]_j = K_t \x_t,
\end{align}
where we construct $K_t$ via
\begin{equation*}
    [K_t]_{ij} = \sum_q \frac{[\x^q_t]_j}{[\x_t]_j}  [K_t^q]_{ij}.
\end{equation*}

\end{proof}



\begin{theorem}
If a game $G$ can be decomposed into $m$ sub-games $\left\{G^q\right\}_{q=1}^{m}$, and the Defender can win all the sub-games, then the Defender can also win the original game $G$.
\end{theorem}
\sg{This theorem needs more assumptions. We need to ensure that Attacker $q_1$'s resource in subgame $q_1$ does not come to subgame $q_2$ to help Attacker $q_2$.}

\daigo{
\begin{theorem}
If the Defender can win all the sub-games for any arbitrary decomposition $\left\{G^q\right\}_{q=1}^{m}$, then Defender can win the original game $G$.
\end{theorem}
\begin{proof}
Let $\pi_Y^q$ denote the $q$-th Attacker policy $\pi_Y^q: Z \mapsto \mathcal{F}$, which is a mapping from the current configuration to the action.
The assumption of the theorem states that for any $\pi_Y^q$, there exists a Defender policy $\pi_X^q$ that ensures
\begin{equation}
    [\x_t^q]_i \geq [\y_t^q]_i, \forall\;i, t.
\end{equation}
This condition ensures $[\x_t]_i\geq [\y_t]_i$ for all $t$.
\end{proof}
}

% \begin{lemma}
% If the Attacker can win the game, then for any decomposition $\left\{G^q\right\}_{q=1}^{m}$, there exists a sub-game that the Attacker can win.
% \end{lemma}
% \begin{proof}
% Suppose the 
% \end{proof}

% \begin{lemma}
% Let $v_t^q=\sum_i \max\{0, [\x_t^q]_i-[\y_t^q]_i\}$ be the utility of sub-game $q$ at time $t$.
% Then the utility of the original game is a linear
% \end{lemma}


\begin{definition}[Split-restricted game]
In a split-restricted game, the Attacker cannot split its resource given its initial distribution $\y_0$.
Formally, at each time step $t$, there exists a partition $\{\nodeset^1_t,\ldots, \nodeset_t^{|\nodeset|}\}$ of the $\nodeset$, such that $\bigcup_{k=1}^{|\nodeset|} \nodeset^k_t=\nodeset$ and $\nodeset^i_t \cap \nodeset^j_t = \emptyset$ for all $i\neq j$.
Further more, at each time step $t$, the resource distribution $\y_t$ follows:
\begin{equation}
    [\y_t]_i = \sum_{j \in \nodeset_t^i} [\y_0]_j.
\end{equation}
\end{definition}
\daigo{Any decomposition can be further decomposed into a ``split-restricted game.''
Why don't we just bake this split-restriction assumption into the original definition of sub-games?}

\begin{theorem}[No incentive to split]
If the Attacker can win the game, then it can win without splitting its resources over multiple battlefields.
\end{theorem}
\todo{Do we want to present anything more general (using the subgame or not)?  Or just say something about future directions? }

\subsubsection{}
Define the winning set of Y as 
\begin{align}
    \polytope_{\text{win}} &= \left\{
    \y_{t+1} \;\vert\; \forall \x_{t+1} \in \RSet(\x_t), ~[\y_{t+1}]_{i} > [\x_{t+1}]_i \text{ for some } i
    \right\}
    \\
    &= \bigcap_{\x \in \RSet(\x_t)} \bigcup_i \left\{
    \y \;\vert\; [\y]_i > [\x]_i
    \right\} 
    \\
    &\supset \bigcap_{\x \in \RSet(\x_t)} \bigcup_i \left\{
    \y \;\vert\; [\y]_i \geq [\x]_i +\epsilon
    \right\} 
    \\
    &\supset \bigcup_i \bigcap_{\x \in \RSet(\x_t)} \left\{
    \y \;\vert\; [\y]_i\geq [\x]_i +\epsilon
    \right\} \\
    &= \bigcup_i \bigcap_{s} 
    \left\{
    \y \;\vert\; [\y]_i\geq [\x^{(s)}_{\RSet(\x_t)}]_i +\epsilon
    \right\}\\
    &= \bigcup_i \left\{
    \y \;\vert\; [\y]_i\geq \max_{s}[\x^{(s)}_{\RSet(\x_t)}]_i +\epsilon
    \right\}
\end{align}
Denote the set of winning node $i$ as 
\begin{equation*}
    \polytope_{\text{win}, i} = \left\{
    \y \;\vert\; [\y]_i\geq \max_{s}[\x^{(s)}_{\RSet(\x_t)}]_i +\epsilon
    \right\}.
\end{equation*}
Then if there exists a node $i$ such that
\begin{equation*}
    \RSet(\y_t) \cap \polytope_{\text{win},i} \ne \emptyset,
\end{equation*}
then the Attacker is guaranteed to win node $i$ at the next time step.
\end{appendix}
